Region Templates: Data Representation and Management for Large-Scale Image Analysis

Distributed memory machines equipped with CPUs and GPUs (hybrid computing nodes) are hard to program because of the multiple layers of memory and heterogeneous computing configurations. In this paper, we introduce a region template abstraction for the efficient management of common data types used in analysis of large datasets of high resolution images on clusters of hybrid computing nodes. The region template provides a generic container template for common data structures, such as points, arrays, regions, and object sets, within a spatial and temporal bounding box. The region template abstraction enables different data management strategies and data I/O implementations, while providing a homogeneous, unified interface to the application for data storage and retrieval. The execution of region templates applications is coordinated by a runtime system that supports efficient execution in hybrid machines. Region templates applications are represented as hierarchical dataflow in which each computing stage may be represented as another dataflow of finer-grain tasks. A number of optimizations for hybrid machines are available in our runtime system, including performance-aware scheduling for maximizing utilization of computing devices and techniques to reduce impact of data transfers between CPUs and GPUs. An experimental evaluation on a state-of-the-art hybrid cluster using a microscopy imaging study shows that this abstraction adds negligible overhead (about 3%) and achieves good scalability.

==> components.tex <==
\subsection{Analytics Framework} \label{sec:analytics-framework}

We have developed an analytics framework to take advantage of 
hybrid computing clusters for common
operation categories, data structures, and processing patterns in 
microscopy image 
analysis applications. The framework consists of three interacting
components. One component manages a library of image analysis
operations~\cite{jamia-insilico,Teodoro:2013:Parco,Teodoro-IPDPS2013,Teodoro-2012-Morph}.
We provide a range of operations, but the library can be 
extended with additional operations.
Operations may be developed with a user-preferred 
language (e.g., OpenCL that supports the execution of a single implementation 
across heterogeneous platforms) as long as it is possible to integrate the 
operations with C++ for proper invocation by the runtime middleware. 
The second component implements the runtime middleware 
for scheduling analysis applications composed of these operations on hybrid 
computing clusters~\cite{Teodoro-IPDPS2012,Teodoro-IPDPS2013}. The third component, 
which is the topic of this paper, provides support for managing data structures 
consumed and produced during analysis executions.  

The middleware layer is designed to support a combination of several processing patterns. 
First, primary image datasets can often be partitioned into tiles or chunks, 
and several categories of operations can be executed on each chunk independently.  This
leads to a bag-of-tasks processing pattern. Second, processing of a single
chunk or a group of chunks can be expressed as a hierarchical coarse-grain
dataflow pattern.  For example, transformation, filtering, mapping, and
segmentation operations can be composed into a pipeline.  Third, several types
of operations such as aggregation and classification can be represented as
MapReduce~\cite{dean04mapreduce} style computations. 
These different computation patterns are supported
in the analytics framework by expressing applications as directed graphs that
specify logical \emph{stages} and the connections, or dependencies, among
the stages.  The logical stages are mapped to data processing operations during
execution. We should note that stages and high-level operations are often built 
from finer-grain functions. The segmentation stage, for instance, is comprised 
of several functions, such as area threshold, distance map computation, and morphological 
reconstruction, which operate on
arrays and objects. This creates a two-level pipeline, in which data processing  
stages such as transformation,
filtering, mapping, and segmentation form the first level, and the pipelines of
finer-grain functions constitute the second level. Hence, a stage may be
mapped to a directed graph of fine-grain \emph{tasks} which are encapsulated in
that stage (Figure~\ref{fig:app}).

Managing interactions among operations is a complex problem 
on systems with nodes equipped with multiple GPUs and CPUs. We have explored 
mechanisms to manage this complexity through dynamic adaptations
and multi-level sc\-he\-du\-ling mechanisms. In our current implementation we employ
function variants coupled with a performance-aware task scheduling (PATS) 
strategy to coordinate the use of CPUs and GPUs~\cite{Teodoro-IPDPS2013}. 
A function variant is defined as a group of functions with the same name, arguments, and result type 
of a high-level, abstract operation. It enables the runtime system to choose the 
appropriate function or functions during execution, allowing multiple computing 
devices (e.g., CPUs and GPUs) to be used concurrently. 
The PATS approach 
maps functions to CPUs and GPUs based on the
functions' estimated GPU speedup values in order to more efficiently 
use the aggregate computing power. The runtime 
system can restrict the execution of an operation to a specific device when only a 
single implementation is available.
Data exchange between pipeline stages and between functions is
carried out via the region template abstraction. This abstraction and the
runtime support for it are described in the next section. 

